Frobenius's last proof

Around about 1917, Issai Schur rediscovered the Rogers-Ramanujan identities, and proved a system of polynomial identities that imply them. Schur wrote that Georg Frobenius (his former advisor) had shown him a simple, direct proof of these polynomial identities. Schur did not see fit to reveal Frobenius's proof, preferring his own rather complicated proof. But it is easy enough to guess what this `simple, direct' proof must have been. As Frobenius died in 1917, we may call this `Frobenius's last proof'.

==> flp_dot_bib <==
\@article{schur:rr,
	author={Issai Schur},
	title={Ein {B}eitrag zur additiven {Z}ahlentheorie and zur {T}heorie der {K}ettenbr\"{u}che},
	journal={S.-B. der Preuss. Akad. Wiss.,
	Phys.-Math. Kl.},
	year={1917},
	pages={302-321},
note={In \emph{Gesammelte Abhandlungen}, vol. 2, pages 117--136}
}

@incollection{gauss:binom,
        author =        {C. F. Gauss},
        title =         {Summatio quarumdam serierum singularium},
        pages =         {2-45},
        booktitle =     {Werke},
        xxxaddress=      {G\"{o}ttingen},
        year =          {1876},
        volume =        {2}
}

@incollection{gauss:100,
        author =        {C. F. Gauss},
        title =         {Hundert {T}heoreme \"{u}ber die neuen {T}ransscendenten},
        pages =         {461-469},
        booktitle =     {Werke},
        xxxaddress =     {G\"{o}ttingen},
        year =          {1876},
        volume =        {3}
}

@book{andrewseriksson,
	author = {George E. Andrews and Kimmo Eriksson},
	title={Integer Partitions},
	year={2004},
	xxxpublisher={Cambridge}
}

